Model Hierarchy Predictive Control of Robotic Systems

This letter presents a new predictive control architecture for high-dimensional robotic systems. As opposed to a conventional Model Predictive Control (MPC) approach to locomotion that formulates a hierarchical sequence of optimization problems, the proposed work formulates a single optimization problem posed over a hierarchy of models, and is thus named Model Hierarchy Predictive Control (MHPC). MHPC is formulated as a multi-phase receding-horizon Trajectory Optimization (TO) problem, and can be implemented using any general multi-phase TO solver. MHPC is benchmarked in simulation on a quadruped, a biped, and a quadrotor, demonstrating control performance on par or exceeding whole-body MPC while maintaining a lower computational cost in each case. A preliminary gap jumping experiment is conducted on the MIT Mini Cheetah with the control policy generated offline, demonstrating the physical validity of the generated trajectories and motivating online MHPC in future work.

==> Sections/HSDDP.tex <==
%[1 page]
Trajectories of the hybrid system can be described by smooth dynamics and reset maps. The reset map takes place only when system state reaches a switching surface and results in a discontinuous jump in state space. Each smooth dynamics is called a mode, and the order it appears is represented by a mode sequence. A hybrid system with a fixed mode sequence can be modeled as follows:
\begin{subequations}\label{eq_hybrid_system}
\begin{align}
    \xi_{k+1} &= \f_i(\xi_k,\ui_k),\label{subeq_dyn}\\ 
     \x^{[i+1]}_0 &= \P_{i}(\xi_{N_{i}}),\label{subeq_reset}\\
     g_{i}(\xi_{N_{i}}) &= 0. \label{subeq_switch}
\end{align}
\end{subequations}
where $\x$ and $\u$ are system state and control, the superscript $[i]$ and subscript $i$ denote mode index, $\f$ and $\P$, respectively, represent smooth dynamics and reset map. The equality constraint~\eqref{subeq_switch} ensures that the reset map takes place at the end of the $i^{\text{th}}$ mode.

The Hybrid-systems DDP (HSDDP) is proposed by \cite{li2020hybrid}, and addresses trajectory optimization (TO) for hybrid systems~\eqref{eq_hybrid_system} using DDP advances. For each mode $i$ of~\eqref{eq_hybrid_system}, we define a cost function
\begin{equation}
    J^{[i]}(\U^{[i]}) = \sum_{k=0}^{N_i - 1} \ell_i(\xi_k, \ui_k) + \phi_i(\xi_{N_i}),
\end{equation}
where $\ell_i$, $\phi_i$ and $N_i$ represent the running cost, the terminal cost, and the length of horizon, respectively, associated with mode $i$, and $\U^{[i]} = [\u^{[i]}_0,\cdots,\u^{[i]}_{N_i-1}]$. 
% The total cost for system~\eqref{eq_hybrid_system} is then defined by
% \begin{equation}
%     J(\bcalU) = \sum_{i=1}^n J^{[i]}(\U^{[i]}),
% \end{equation}
% where $n$ denotes the total number of modes, and $\bcalU = [\U^{[1]},\cdots,\U^{[n]}]$. 
A TO for hybrid systems~\eqref{eq_hybrid_system} can be formulated as follows 
\begin{subequations}\label{eq_hybridTO}
\begin{IEEEeqnarray}{cll}
\IEEEeqnarraymulticol{2}{l}{\min_{\bcalU} \ \ \sum_{i=1}^n J^{[i]}(\U^{[i]})}\\
    \text{subject~to} \ \ & \eqref{subeq_dyn}, \eqref{subeq_reset}\\ 
     & \eqref{subeq_switch}\\
     &h_i(\xi_k,\ui_k)\geq \mathbf{0}, \label{subeq_ineq}
\end{IEEEeqnarray}
\end{subequations}
where $\bcalU = [\U^{[1]},\cdots,\U^{[n]}]$ and $h$ represents inequality constraints such as torque limits.

The HSDDP attacks ~\eqref{eq_hybridTO} by converting it into an unconstrained optimization problem using Augmented Lagrangian (AL) and Reduced Barrier method (ReB). A Lagrangian-like function at mode $i$ could be constructed as follows
\begin{multline}\label{eq_mode_Lagrangian}
    \calL^{[i]}(\U^{[i]},\lambda_i,\sigma_i,\delta_i) = \sum_{k=0}^{N_i - 1} \underbrace{\ell_i(\xi_k, \ui_k) + B_{\delta_i}\big(h_i(\xi_k,\ui_k) \big)}_{L_i(\xi_k, \ui_k)} \\ 
    +\underbrace{\phi_i(\xi_{N_i}) + \left(\frac{\sigma_i}{2}\right)^2 g_i(\xi_{N_i}) + \lambda_i g_i^2(\xi_{N_i})}_{\Phi_i(\xi_{N_i})},
\end{multline}
where $\lambda_i$ and $\sigma_i$ are Lagrange multiplier and penalty coefficient, respectively, and $B_{\delta_i}$ is a reduced Barrier function \cite{hauser2006barrier,li2020hybrid} parameterized by the relax parameter $\delta_i$. The Lagrangian-like function for the entire system~\eqref{eq_hybrid_system} is then
\begin{equation}\label{eq_Lagrangian}
    \calL(\bcalU,\blambda, \bsigma, \bdelta) =  \sum_{i=1}^n \calL^{[i]}(\U^{[i]},\lambda_i,\sigma_i,\delta_i),
\end{equation}
where $\blambda = [\lambda_1,\cdots,\lambda_n]$, $\bsigma$ and $\bdelta$ are similarly defined. 

The reformulated unconstrained optimization problem is stated as follows
\begin{subequations}\label{eq_hybridTO_unconstr}
\begin{IEEEeqnarray}{cll}
\IEEEeqnarraymulticol{2}{l}{\min_{\bcalU} \ \ \calL(\bcalU,\blambda, \bsigma, \bdelta)}\\
    \text{subject~to} \ \ & \eqref{subeq_dyn}, \eqref{subeq_reset}.
\end{IEEEeqnarray}
\end{subequations}
The HSDDP sovles~\eqref{eq_hybridTO_unconstr} with fixed $\blambda, \bsigma, \bdelta$ using DDP, and employs an outer loop to iteratively reset their values until all constraints are satisfied. The update equations are as follows
\begin{equation}
    \bsigma \leftarrow \beta_{\sigma}\bsigma, \ \ 
    \blambda \leftarrow \blambda + \bsigma \circ\g, \ \   
    \bdelta \leftarrow \beta_{\delta}\bdelta, \label{eq_update}
\end{equation}
where $\beta_{\sigma}>0$ and $0<\beta_{\delta}<1$ are update parameters, the vector $\g$ concatenates all $g_{i}(\xi_{N_{i}})$ and the operator $\circ$ denotes element-wise product. 

Care must be taken when solving~\eqref{eq_hybridTO_unconstr} with DDP due to the discontinuous jump caused by~\eqref{subeq_reset}. This is addressed in HSDDP by employing an impact-aware step. Denote $V(\xi_k)$ the optimal cost-to-go evaluated at $\xi_k$. 
% According to Bellman's principle of optimality, for $0\leq k<N_i$
% \begin{equation}
%     V(\xi_{k}) = \min_{\ui_k}\ \Big\{\ell_i(\xi_k, \ui_k) + V\Big(\f_i(\xi_k, \ui_k) \Big)\Big\},
% \end{equation}
% and at $k = N_i$,
% \begin{equation}
%     V(\xi_{N}) = \ \ \phi_i(\xi_{N_i}) + V\Big(\P_i(\xi_N) \Big).
% \end{equation}
The variation of $V(\xi_k)$ along a nominal trajectory under perturbation $(\delta\xi_k,\delta\ui_k)$ is approximated to the second order as follows
\begin{equation}\label{eq_value_func_approx}
    \delta V(\delta\xi_k) \approx \frac{1}{2}(\delta\xi_k)^\top\Si_k\delta\xi_k + (\bsi_k)^\top\delta\xi_k + \si_k,
\end{equation}
where $\Si_k$, $\bsi_k$ and $\si_k$ respectively, represent the hessian, gradient, and scalar terms. The HSDDP recursively computes these terms for all $k$ and $i$ by performing a backward sweep. For $0\leq k<N_i$ at mode $i$, the recursive equations are
\begin{subequations}\label{eq_value_update_smooth}
\begin{align}
    s &= s'  + \frac{1}{2}\qsu^T\qsuu^{-1}\qsu, \label{eq_scalar}\\
    \s &= \qsx - \qsux^T\qsuu^{-1}\qsu, \label{eq_gradient}\\
    \S &= \qsxx - \qsux^T\qsuu^{-1}\qsux \label{eq_hessain},
\end{align}
\end{subequations}
where 
\begin{subequations}\label{eq_Qs}
\begin{align}
    \qsx &= \Lx + \fx^\top\s',\\
    \qsu &= \Lu + \fu^\top\s',\\
    \qsxx &= \Lxx + \fx^\top\S'\fx + \s' \cdot  \fxx,\\
    \qsuu &= \Luu + \fu^\top\S'\fu + \s' \cdot  \fuu,\\
    \qsux &= \Lux + \fu^\top\S'\fx + \s' \cdot \fux,
\end{align}
\end{subequations}
in which the subscripts indicate the partial derivatives and the prime indicates the next time step. Note that $\fxx$, $\fuu$ and $\fux$ generally are tensors. The notation `$\cdot$' denotes matrix-tensor multiplication. At $k=N_i$, the recursive equations are
\begin{subequations}\label{eq_value_update_jump}
\begin{align}
    s &= s',\\
    \s &= \Phi_{\x} + \P_{\x}^\top\s',\\
    \S & = \Phi_{\x\x} + \P_{\x}^\top\S' \P_{\x}.
\end{align}
\end{subequations}
Note that in eq~\eqref{eq_value_update_jump}, the prime indicates the next step is at $k=0$ of mode $i+1$. The value function approximation thus obtained are used to construct the control policy
\begin{equation}\label{eq_optdu}
     \delta\u^* = -\qsuu^{-1}(\qsu + \qsux\delta\x) \equiv \bkappa + \mathbf{K}\delta\x.
\end{equation}
A line search method and a regularization step are typically performed with~\eqref{eq_optdu} to ensure cost reduction. A pseudo code for HSDDP algorithm is shown in Algorithm \ref{alg_HSDDP}. The readers are referred to \cite{li2020hybrid} for a detailed description of HSDDP.

\begin{algorithm}[t]
    \caption{HSDDP Algorithm}
    \label{alg_HSDDP}
    \begin{algorithmic}[1] 
        \State Initialize $\blambda,\bsigma, \bdelta$.
        \While {$\norm{\g}_2>$ tol.}
        \State Minimize $\calL(\bcalU,\blambda,\bsigma, \bdelta)$ using DDP (carry out eq~\eqref{eq_value_update_jump} at mode transition in backward sweep).
        \State Compute $g_{c_i}(\x^-_{N_i})$.
        \State Update $\blambda,\bsigma, \bdelta$ using eq~\eqref{eq_update}
        \EndWhile
    \end{algorithmic}
\end{algorithm}


